Quasi-likelihood analysis of an ergodic diffusion plus noise

We consider adaptive maximum-likelihood-type estimators and adaptive Bayes-type ones for discretely observed ergodic diffusion processes with observation noise whose variance is constant. The quasi-likelihood functions for the diffusion and drift parameters are introduced and the polynomial-type large deviation inequalities for those quasi-likelihoods are shown to see the convergence of moments for those estimators.

==> preamble.tex <==
\usepackage[a4paper,top=3cm,bottom=3cm,left=2.5cm,right=2.5cm,marginparwidth=1.75cm]{geometry}

% maketitle
\usepackage[UKenglish]{babel}

% math fonts and symbols
\usepackage{amsfonts,amsmath,amsthm,amssymb} % \text and \mathbb command
\usepackage[foot]{amsaddr}
\usepackage{mathrsfs} % script type font
\usepackage{stmaryrd} % new bracket

% Bernoulli Journal
\RequirePackage[OT1]{fontenc}
\usepackage{natbib}

\RequirePackage[colorlinks,citecolor=black,urlcolor=blue]{hyperref}

% others
\usepackage{comment} % commenting out multiple lines
\usepackage{graphicx} % graphics
\usepackage{setspace}
\usepackage{subcaption}
\usepackage{color}

\allowdisplaybreaks[1]
%\setlength\parindent{15pt}

\newcommand{\R}{\mathbf{R}}
\newcommand{\N}{\mathbf{N}}
\newcommand{\lm}[2]{\bar{#1}_{#2}}

\newtheorem{theorem}{Theorem}%[subsection]
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}

\theoremstyle{remark}
\newtheorem{remark}{Remark}

